ExtraNeRF: Visibility-Aware View Extrapolation of Neural Radiance Fields with Diffusion Models

We propose ExtraNeRF, a novel method for extrapolating the range of views handled by a Neural Radiance Field (NeRF). Our main idea is to leverage NeRFs to model scene-specific, fine-grained details, while capitalizing on diffusion models to extrapolate beyond our observed data. A key ingredient is to track visibility to determine what portions of the scene have not been observed, and focus on reconstructing those regions consistently with diffusion models. Our primary contributions include a visibility-aware diffusion-based inpainting module that is fine-tuned on the input imagery, yielding an initial NeRF with moderate quality (often blurry) inpainted regions, followed by a second diffusion model trained on the input imagery to consistently enhance, notably sharpen, the inpainted imagery from the first pass. We demonstrate high-quality results, extrapolating beyond a small number of (typically six or fewer) input views, effectively outpainting the NeRF as well as inpainting newly disoccluded regions inside the original viewing volume. We compare with related work both quantitatively and qualitatively and show significant gains over prior art.

==> sec/3_background.tex <==
\section{Background}
\color{mengli_wo_gpt}{
\subsection*{Neural Radiance Fields}
Neural Radiance Fields (NeRFs)~\cite{mildenhall2020nerf} represent a novel implicit neural field representation, primarily designed for 3D scenes and objects. These models are typically trained using multi-view image datasets. At its core, NeRF consists of two fundamental components:

(i) A learnable field, denoted as $f_{\theta}:(x, d) \rightarrow (c, \sigma)$, which takes as input a 3D coordinate, $x \in \mathbb{R}^3$, and a view direction, $d \in \mathbb{S}^2$, and maps them to a color, $c \in \mathbb{R}^3$, and density, $\sigma \in \mathbb{R}^+$. The mapping is governed by a set of learnable parameters denoted as $\theta$.

(ii) A rendering operator responsible for generating color and depth information for each pixel in a given view. This rendering operator employs the classical volume rendering integral~\cite{max1995optical}. Specifically, a ray, denoted as $r$, is discretized into $N$ evenly sections spanning from $t_n$ (the near bound) to $t_f$ (the far bound). These sections are defined by sampled values of $t_i$ within the $i$-th section. The estimated color for a particular ray is then computed as follows:

\begin{equation}
\label{eq:volumetric-rendering}
\hat{C}(r) = \sum_{i = 1}^{N} T_i(1 - \exp(-\sigma_i \delta_i))c_i,
\end{equation}

Here, $T_i = \exp(-\sum_{j = 1}^{i - 1} \sigma_j \delta_j)$ represents the transmittance, $\delta_i = t_{i + 1} - t_i$ is the section's length, and $c_i$ and $\sigma_i$ denote the color and density at $t_i$. By replacing $c_i$ with $t_i$ in Equation~\ref{eq:volumetric-rendering}, one can estimate depth, denoted as $\hat{D}(r)$.
}



==> sec/X4_oldmethod.tex <==
\section{Method}
\textcolor{mengli_wo_gpt}
Our primary design goals is to extrapolate views beyond the input viewpoints: user can see plausible and view-consistent content beyond the captured data. To this end, we propose a pipeline consists of 3 stages to fulfill the requirement. This includes data-preprocessing(sec.~\ref{subsec:data-preproc}), scene reconstruction(sec.~\ref{subsec:reconstruction}), content hallucination(sec.~\ref{subsec:cont-hallucinate}), and content enhancement(sec.~\ref{subsec:cont-enhance}).
\newline

\subsection{Data pre-processing} \label{subsec:data-preproc} 
The input to our reconstruction algorithm is a set of captured photos $\{I_i\}_{i=1}^{n}$ and the associated viewpoint matrices $\{\Pi_i\}_{i=1}^{n}$. Given these as input data, we exploit a state-of-the-art reconstruction method \cite{sparf2023} to get a 3D reconstruction. From there, we could render a set of depth maps $\{D^{preproc}_i\}_{i=1}^{n}$ corresponded to the input images $\{I_i\}_{i=1}^{n}$.(see Figure X)

\subsection{Scene reconstruction} \label{subsec:reconstruction}
Given the data from sec.~\ref{subsec:data-preproc}, we fit a highly efficient and powerful variant of NeRF~\cite{mueller2022instant} governed by parameter $f_{\theta}$ and supervised by objective eq.~\ref{eq:objective_stage1}. 
\begin{align} \begin{split} \label{eq:objective_stage1}
    L_{recon} = \mathbb{E}_{r\sim\mathcal{R}}[&||\hat{C}(r)-C_{GT}(r)||^2_2 + L_{distortion}(r) \\
    + & ||\hat{D}(r)-D^{preproc}(r)||^2_2 + L_{hash-decay}]
 \end{split} \end{align}
,where $\mathcal{R}$ is the set of rays aligned with pixels in $\{I_i\}_{i=1}^{n}$, $C_{GT}$ and $D^{preproc}$ is the ground-truth color and preprocess depth at ray $r$, and $L_{distortion}$~\cite{barron2021mip} and $L_{hash-decay}$~\cite{barron2023zip} are losses applied on ray $r$ to reduce floating artifact. Besides, we applied a gradient scaling technique~\cite{philip2023floaters} to further reduce the floater.
\subsection{Content Hallucination} \label{subsec:cont-hallucinate}
A NeRF parameterized by $f_\theta$ encode 3-D content observed from photos $\{I_i\}_{i=1}^{n}$(see. sec.~\ref{subsec:reconstruction}) can rendering decent images given viewpoints within the range of $\{\Pi_i\}_{i=1}^{n}$. Yet, our goal is to further render images given viewpoints beyond this range. To achieve it, two more things are required. A camera trajectory consists of viewpoints beyond the range of $\{\Pi_i\}_{i=1}^{n}$, and 3-D content that is unobserved from $\{\Pi_i\}_{i=1}^{n}$.\\
User can create a new circle camera trajectory easily by specifying two parameters only, center viewpoint matrices $\Pi_{center}$ and the radius of the circle $rad$. Next, we evenly sample $m$ viewpoints $\{\Pi^{virtual}_i\}_{i=1}^{m}$ on this circle trajectory. As long as the radius is larger than the range of input viewpoints $\{\Pi_i\}_{i=1}^{n}$, area unobserved from $\{\Pi_i\}_{i=1}^{n}$ is revealed now. Following a series of works originated from~\cite{poole2022dreamfusion}, in which 3d content is generated under the guidance of natural image prior from a diffusion model~\cite{rombach2022high, shi2020improving, saharia2022photorealistic}, we can hallucinate 3d content in the unobserved area revealed from viewpoints $\{\Pi^{virtual}_i\}_{i=1}^{m}$. Besides, as the NeRF $f_\theta$ already encode part of real content from $\{I_i\}_{i=1}^{n}$, we choose to use inpainting variants of ~\cite{rombach2022high}, which preserves observed real content and introduces image prior consistent seamlessly and consistently. \\
As we're going to use inpainting variant of diffusion model, denoted as $\Phi$, identifying those unobserved area in 2D images rendered from viewpoints $\{\Pi^{virtual}_i\}_{i=1}^{m}$ is required. We develop an algorithm to volumetric render unobserved area from NeRF $f_\theta$. \\
\subsubsection{2-D Mask of unobserved area} \label{subsubsec:2d-unobserved-mask}
In volumetric rendering, we can use transmittance $T$ to represent the visibility of a 3-D point. Hence, given a point $p$ on a ray $r$ from a pixel in image corresponding to $\{\Pi^{virtual}_i\}_{i=1}^{m}$, we can calculate their transmittances $T$  according to input viewpoints $\{\Pi_i\}_{i=1}^{n}$ using eq.~\ref{eq:volumetric-rendering}. Besides, a point $p$ lies outside camera frustum of viewpoints $\{\Pi_i\}_{i=1}^{n}$ is not visible, and we let $T = 0$ for those points. We then define the extent of visibility $v$ by choosing the $k$-th largest transmittance $T$. Here, $k$ indicates the number of viewpoints $\{\Pi_i\}_{i=1}^{n}$ that can observe the point $p$. We set $k=2$ as 2-view geometry is the minimum requirement for reliable 3-D reconstruction. Next, by replacing $c_i$ in eq.~\ref{eq:volumetric-rendering} with $v$, we can render the visibility masks from viewpoints $\{\Pi^{virtual}_i\}_{i=1}^{m}$. Finally, by taking the inverse of this visibility masks and set a threshold $th_{vis}$, we highlight those unobserved area in 2D images, denoted as $\{M^{virtual}_i\}_{i=1}^m$\\. Following the same way, we identify the mask region in input images $\{I_i\}_{i=1}^{n}$ that is visible by exact one of the viewpoints $\{\Pi_i\}_{i=1}^{n}$ only, denoted as $\{M_i\}_{i=1}^n$.
\subsubsection{Supervision from inpainting module} \label{subsubsec:supervision-from-inpainting}
We randomly sample a viewpoint $\Pi^{virtual}$ from $\{\Pi^{virtual}_i\}_{i=1}^{m}$ for each iteration, and render the corresponding image $I^{virtual}$, depth map $D^{virtual}$ and mask $M^{virtual}$ from $\Pi^{virtual}$ with $f_\theta$. By taking $M^{virtual}$,  $I^{virtual}$, and a noise level $t_{noise}\sim[0.02, 0.98]$ as input, the inpainting diffusion model $\Phi$ output a denoised inpainted image $I^{inpaint}$. This $I^{inpaint}$ can be used to supervise $f_\theta$ through the pixels in $M^{virtual}$ (see Eq.~\ref{eq:objective_stage2_synpix_inpaint_pho}). 
\begin{align} \begin{split} \label{eq:objective_stage2_synpix_inpaint_pho}
    L_{pho}^{inpaint} = &\mathbb{E}_{r\sim\mathcal{\widetilde{R}}}[|\hat{C}(r)-C^{inpaint}(r)|]
\end{split} \end{align}
,where $\widetilde{R}$ is the set of rays corresponding to pixels in $M^{virtual}$, and $C^{inpaint}$ is the color of inpainted color in $I^{inpaint}$.
In addition to color supervision, geometry supervision has shown its effectiveness during recent works~\cite{tang2023makeit3d, mirzaei2023reference, sun2023dreamcraft3d} of 3-D content generation. Thus, we also adopt geometry supervision using depth map $D^{inpaint}$ obtained from a depth completion module $\Psi$. Specifically, the depth completion module takes $I^{inpaint}$, $D^{virtual}$, and $M^{virtual}$ as input, and output $D^{inpaint}$. Then, we introduce geometry supervision using Eq.~\ref{eq:objective_stage2_synpix_inpaint_depth}.
\begin{align} \begin{split} \label{eq:objective_stage2_synpix_inpaint_depth}
    L_{depth}^{inpaint} = &\mathbb{E}_{r\sim\mathcal{\widetilde{R}}}[|\hat{D}(r)-D^{inpaint}(r)|]
\end{split} \end{align}
Besides using Eq.~\ref{eq:objective_stage2_synpix_inpaint_pho} and ~\ref{eq:objective_stage2_synpix_inpaint_depth} to create content in $f_\theta$, we also apply Eq.~\ref{eq:objective_stage1} to preserve the reconstruction in the observed area. We shown the result in fig.~\ref{}.

Although the synthesized content is plausible in fig.~\ref{}, it still has some artifact(i.e. rubber sheeting artifact, and blurred detail). We describe reasons of and solutions to them in sec.~\ref{subsubsec:rubber-sheet-artifact} and sec.~\ref{subsec:blurred-detail}.
\subsubsection{Ambiguity in inpainted object boundary} \label{subsubsec:rubber-sheet-artifact}
Dis-occlusion occurs when something is visible from virtual viewpoints $\{\Pi^{virtual}_i\}_{i=1}^{m}$ but blocked from input viewpoints $\{\Pi_i\}_{i=1}^{n}$ by other objects. Synthesize content of dis-occlusion that is observed from $\{\Pi^{virtual}_i\}_{i=1}^{m}$ via 2-D image inpainting could be ambiguous. The model cannot certainly identify a consistent boundary of foreground and dis-occluded background when doing 2-D inpainting from various viewpoints$\{\Pi^{virtual}_i\}_{i=1}^{m}$. This issue becomes more significant when the diffusion model is adopted. As we use different noise map in different training iterations, the boundary in the inpainted image $I^{inpaint}$(see fig.~\ref{}) is also different. Thus, the supervision that NeRF $f_\theta$ received from $I^{inpaint}$ between different viewpoints or iterations are inconsistent. The result is a mixture of foreground and background content in the dis-occlusion when render via NeRF $f_\theta$ from $\{\Pi^{virtual}_i\}_{i=1}^{m}$.(see fig.~\ref{})\\
An intuitive way is to teach the diffusion model to inpaint dis-occluded background rather than foreground content~\cite{jampani2021slide, xiang20233d}. We achieve this by fine-tuning our inpainting model $\Psi$ with dis-occlusion masks corresponding to $\{I_i\}_{i=1}^{n}$ using algorithm in sec.~\ref{subsubsec:2d-unobserved-mask}(see fig.~\ref{}). Since pixels in dis-occlusion mask is aligned with those background content near foreground object, the fine-tuned model $\Psi_{disocc}$ learns to inpaint background with this kind of data. By replacing $\Psi_{disocc}$ with $\Psi$, we obtain $I^{inpaint}$ that has less ambiguity of object boundary in disocclusion region.

\subsection{Absence of contents in detail} \label{subsec:blurred-detail}
When the level of detail in the unobserved content is high, it is hard to hallucinate these detail consistently across different viewpoints and different noise maps. Thus, the hallucinated content from sec.~\ref{subsec:cont-hallucinate} still misses detail. \textcolor{note}{These words could be put in the related works section? A series of methods~\cite{} suggest to sample(inpaint) from the diffusion model once and set that result as the supervision for the remaining training process of NeRF $f_\theta$. However, it is hard to guarantee a random sample of inpainted result is plausible among different viewpoints. Also, using only one sample from the diffusion model as the supervision prevents the NeRF $f_\theta$ to receive a comprehensive natural image prior from the diffusion model. Additionally, another series of methods~\cite{wang2023prolificdreamer, sun2023dreamcraft3d} suggest to anneal the level of noise $t_noise$ injected into the diffusion model gradually(i.e. noise annealing). However, the amount of detailed enhanced by of this method is still limited(see fig.~\ref{}).}
In contrast the above methods, we teach the diffusion model $\Psi$ to enhance the detail by fine-tuning it with pairs of gaussian-blurred images vs. ground-truth clear images$\{I_{i=1}^{n}\}$(see fig.~\ref{}). This fine-tuned model $\Psi_{enhance}$ can be adopted to enhance a rendered image $I^{virtual}$ and get the enhanced image $I^{enhance}$(see fig.~\ref{}). By replacing $C^{inpaint}(\cdot)$ and $D^{inpaint}(\cdot)$ in Eq.~\ref{eq:objective_stage2_synpix_inpaint_pho} and~\ref{eq:objective_stage2_synpix_inpaint_depth} with $C^{enhance}(\cdot)$ and $D^{enhance}(\cdot)$ respectively, we get Eq.~\ref{eq:objective_stage2_synpix_enhance_pho} and~\ref{eq:objective_stage2_synpix_enhance_depth}. Following sec.~\ref{subsec:cont-hallucinate}, we use Eq.~\ref{eq:objective_stage2_synpix_enhance_pho}, ~\ref{eq:objective_stage2_synpix_enhance_depth}, and~\ref{eq:objective_stage1} to enhance the detailed of content in $f_\theta$.
\begin{align} \begin{split} \label{eq:objective_stage2_synpix_enhance_pho}
    L_{depth}^{enhance} = &\mathbb{E}_{r\sim\mathcal{\widetilde{R}}}[|\hat{D}(r)-D^{enhance}(r)|]
\end{split} \end{align}
\begin{align} \begin{split} \label{eq:objective_stage2_synpix_enhance_depth}
    L_{depth}^{enhance} = &\mathbb{E}_{r\sim\mathcal{\widetilde{R}}}[|\hat{D}(r)-D^{enhance}(r)|]
\end{split} \end{align}

However, in practice, when using $\Psi_{enhance}$ to supervise NeRF $f_\theta$, any slight color mismatch between rendered images $I^{virtual}$ and $I^{enhance}$ is accunlated in $f_\theta$ and results in serious color deviation after several iterations(see fig.~\ref{}). Unlike inpainting module $\Psi_{inpaint}$, which re-paint the content in masked region of rendered image $I^{virtual}$, $\Psi_{enhance}$ tend to preserve or enhance the content with mis-matched color in $I^{virtual}$. To deal with it, we teach $\Psi_{enhance}$ to enhance detail and correct the mismatched color simultaneously. We achieve this by fine-tune $\Psi_{enhance}$ again with samples that take mis-matched color in masked image as input and ground-truth image ${I_i}_{i=1}^n$ as output. There are two ways to generate images with mis-mathced color in masked region. \\
\heading{Color jittering}
By jittering the brightness, contrast, saturation, and hue of input images in the mask region, we get the augmented data with mis-matched color. This augmentation is easy to implement, but it is hard to find a unify jittering parameters for all the examples(see.fig.~\ref{]}).\\
\heading{Accumulated color shifting}
As the goal is to correct the mis-matched color in the rendered image $I^{virtual}$ during training, the most efficient way is to use these images $I^{virtual}$ with mis-mathced color as the augmented data. However, we do not have corresponding ground-truth image of $I^{virtual}$. In another word, if we can accumulate mis-mathced color in images from $\{\Pi_i\}_{i=1}^{n}$, we can get training pairs of image with and without mis-matched color. To achieve this, we train another NeRF $f_{\theta^{\prime}}$ using objectives Eq.~\ref{eq:objective_stage2_synpix_enhance_pho}, ~\ref{eq:objective_stage2_synpix_enhance_depth}, and~\ref{eq:objective_stage1} but reduce the span of set $\mathcal{R}$ in Eq.~\ref{eq:objective_stage1} to $\mathcal{R^{\prime}}$. The elements in $\mathcal{R^{\prime}}$ is the ray of pixel in the cropped version of $\{I_i\}_{i=1}^n$. Thus, those pixels of $\{I_i\}_{i=1}^n$ that lie outside the cropped boundary do not receive the supervision to preserve the reconstruction content anymore and the corresponding colors are deviate gradually(see fig.~\ref{}). As a result, we generate input-target pair using these kind of augmented data and ground-truth images ${I_i}_{i=1}^n$. 
Using the augmented data collected via above two methods along with the gaussian-blurred images, we fine-tune model $\Psi$ and get $\Psi_{enhance^+}$ which can not only enhance detail but also correct the deviated color. By replacing $C^{enhance}$ and $D^{enhance}$ with $C^{enhance^+}$ and $D^{enhance^+}$ respectively, we get Eq.~\ref{eq:objective_stage2_synpix_enhance+_pho} and~\ref{eq:objective_stage2_synpix_enhance+_depth}. Finally, we use Eq.~\ref{eq:objective_stage2_synpix_enhance+_pho}, ~\ref{eq:objective_stage2_synpix_enhance+_depth}, and ~\ref{eq:objective_stage1} to enhance the absent detail in $f_\theta$.
\begin{align} \begin{split} \label{eq:objective_stage2_synpix_enhance+_pho}
    L_{depth}^{enhance^+} = &\mathbb{E}_{r\sim\mathcal{\widetilde{R}}}[|\hat{D}(r)-D^{enhance^+}(r)|]
\end{split} \end{align}
\begin{align} \begin{split} \label{eq:objective_stage2_synpix_enhance+_depth}
    L_{depth}^{enhance^+} = &\mathbb{E}_{r\sim\mathcal{\widetilde{R}}}[|\hat{D}(r)-D^{enhance^+}(r)|]
\end{split} \end{align}




==> src/fig/dist2psnr.tex <==
\begin{figure}[h] 
\centering
\vspace{-3mm}
% trim={left bottom right top}
\includegraphics[width=1.0\linewidth, trim={0 0 0 0}, clip]{src/images/distance_2_psnr.png}
\vspace{-8mm}
\caption{Extrapolation distance performance on ``horns'' (Fig.~\textcolor{red}{1}).}
\vspace{-3mm}
\label{fig:dist2psnr}
\end{figure}

==> src/fig/rebuttal_method_overview.tex <==
\begin{figure}[h] 
\centering
\vspace{-5mm}
\includegraphics[width=0.89\linewidth, trim={0 0 0 0}, clip]{src/images/rebuttal_method_overview.png}
\vspace{-4mm}

\caption{\centering Revised method overview (will be two columns wide)\newline Zoom in for better visualization}
\vspace{-5mm}
\label{fig:revise_method_overview}
\end{figure}

==> src/tab/quantitative_llff_freenerf_rebutt.tex <==
\begin{table}[h]
%\caption{\tb{Ablation study on color inpainting.} Using color inpainting model gives better perceptual quality, and our dilation heuristic further boosts the performance. \blue{blue}: results in disocculded regions.}%
% \vspace{-3mm}
\centering
\caption{Comparison to FreeNeRF.}%
% \vspace{-3mm}
\label{tab:quantitative_llff_freenerf_rebutt}
\centering
%\resizebox{\linewidth}{!}{
\small
\setlength{\tabcolsep}{1pt}
\begin{tabular}{l|ccccc}
% \toprule
    Methods        &   PSNR $\uparrow$ &   SSIM $\uparrow$&   LPIPS $\downarrow$ & KID $\downarrow$ & MUSIQ $\uparrow$\\ 
\midrule
    FreeNeRF       &   20.16           &   0.663         &   0.329  & 0.0203 & 39.51        \\ %\hline
    Ours           & \textbf{20.76}    & \textbf{0.688}   & \textbf{0.269} & \textbf{0.0154} & \textbf{54.13}\\
% 0.0203 39.51
% \bottomrule
\end{tabular}
\end{table}

==> src/tab/quantitative_llff_rebutt.tex <==
\begin{table}[htb]

\centering
\caption{Quantitative comparison on LLFF dataset.}%
\vspace{-3mm}~
\label{tab:quantitative_llff_rebutt}

\centering
%\resizebox{\linewidth}{!}{
\small
\setlength{\tabcolsep}{1pt}

\scalebox{0.9}{
\begin{tabular}{lccccc}
\toprule
    Metrics        &   ~Sparf~ &   ~DiffusioNeRF~ &   ~SPIn-NeRF~ & ~FreeNeRF~  & ~Ours~\\ 
\midrule
    PSNR $\uparrow$ &   20.38           &   19.94         &   20.40  & 20.16 & \textbf{20.76}        \\ %\hline
    \textcolor{blue}{$\text{PSNR}_{disocc}$ $\uparrow$} &   \textcolor{blue}{16.26}           &   \textcolor{blue}{15.02}         &   \textcolor{blue}{16.30}  & \textcolor{blue}{15.50} & \textcolor{blue}{\textbf{17.01}}        \\ %\hline    
    SSIM $\uparrow$ &    0.650    & 0.683   & 0.672 & 0.663 & \textbf{0.688}\\
    \textcolor{blue}{$\text{SSIM}_{disocc}$ $\uparrow$} &    \textcolor{blue}{0.435}    & \textcolor{blue}{0.413}   & \textcolor{blue}{0.430} & \textcolor{blue}{0.411} & \textcolor{blue}{\textbf{0.490}}\\    

\bottomrule
\vspace{-5mm}
\end{tabular}
}
\end{table}


